Correlated bandits or: How to minimize mean-squared error online

While the objective in traditional multi-armed bandit problems is to find the arm with the highest mean, in many settings, finding an arm that best captures information about other arms is of interest. This objective, however, requires learning the underlying correlation structure and not just the means of the arms. Sensors placement for industrial surveillance and cellular network monitoring are a few applications, where the underlying correlation structure plays an important role. Motivated by such applications, we formulate the correlated bandit problem, where the objective is to find the arm with the lowest mean-squared error (MSE) in estimating all the arms. To this end, we derive first an MSE estimator, based on sample variances and covariances, and show that our estimator exponentially concentrates around the true MSE. Under a best-arm identification framework, we propose a successive rejects type algorithm and provide bounds on the probability of error in identifying the best arm. Using minmax theory, we also derive fundamental performance limits for the correlated bandit problem.

==> proof_sketch.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection*{Proof of Proposition \ref{prop:mse-conc} \textit{(Sketch)}}
The MSE estimate in \eqref{eq:mse-est-i} involves sample variances and sample correlation coefficients, and hence, MSE concentration requires each of these quantities to concentrate. While one can use Bernstein's inequality (see Lemma \ref{lemma:subexp-conc} in the appendix) for handling sample variance, a finite sample concentration bound for sample correlation coefficient does not exist, to the best of our knowledge. We fill this gap in the result below. 
\begin{lemma}%\textbf{\textit{(Concentration of sample correlation coefficient)}} 
\label{lemma:rho-conc-main}
For independent Gaussian rvs $X_{i}, \ i=1,\ldots,n$, with mean zero and covariance matrix $\Sigma$ as defined in \eqref{eq:gauss-covar} and with $\hat\sigma_i^2$, $\hat\rho_{ij}$ formed from $n$ samples using \eqref{eq:rhohat}, for any $i,j=1,\ldots,K$, and for any $\epsilon \in [0,\eta]$,  we have 
\begin{align*}
 & \P \left (  \left|\hat\rho_{ij} -  \rho_{ij} \right| > \epsilon   \right) \\
&\le 26\exp \left ( - \frac{n}{8} \frac{1}{36(1+\eta)} \min\left( \frac{l \epsilon}{3}, \left ( \frac{l \epsilon}{3} \right)^2\right) \right), 
\end{align*} 
where $l$ is a positive constant satisfying $l \le \sigma_i^2 \le 1$, $\forall i$.
\end{lemma}
The proof is found in Appendix \ref{sec:proofs-mse-conc}. 
We now provide a sketch of the proof of Proposition \ref{prop:mse-conc}.
\begin{proof}\textbf{\textit{(Sketch)}}
 \ \\
We prove the proposition for $i=1$, but the analysis below holds in general. 
Consider the event $\C = \left \{ \sigma_i^2 - \epsilon \leq {\hat \sigma}_{i}^2 \leq  \sigma_{i}^2 + \epsilon, i=1,\ldots,K,  \right.$
$\left.\textrm{ and } \rho_{1j} - \epsilon \le \hat\rho_{1j} \le \rho_{1j}+ \epsilon,  \textrm{ for } j=2,\ldots,K \right\}$.
Then, from the lemma above on sample correlation coefficient concentration and Lemma \ref{lemma:subexp-conc} in the appendix, we have\\[0.5ex]
\centerline{$ \Prob{ \C^c} \le 28K\exp \left ( - \frac{n}{8} \frac{1}{36(1+\eta)} \min\left( \frac{l \epsilon}{3}, \left ( \frac{l \epsilon}{3} \right)^2\right) \right).$}
We shall bound the tail probability $\Prob{ \hat\cE_{1} - \cE_{1} > \epsilon}$ on the event $\C$ and use the bounds on the probability of $\C^c$ to arrive at an unconditional bound on the aforementioned tail probability.
Using an union bound, we have
\begin{align*}
 &  \P \left (  \hat\cE_1  - \cE_1 \geq  \epsilon \! \right ) \le \P \left ( \hat\cE_1  - \cE_1 \geq \epsilon, \C \! \right ) + 
 \P \left ( \C^c \! \right ) \\
 %%%%%%%%
 & \leq \P \left ( {\hat \sigma}_{2}^2 \left ( 1 - \hat\rho_{12}^2  \right ) - { \sigma}_{2}^2 \left ( 1 - \rho_{12}^2  \right )  \geq \frac{\epsilon}{(K-1)}, \C  \right ) \\
&    + \sum \limits_{p=3}^{K}  \P \left (  {\hat \sigma}_{p}^2 \left ( 1 - \hat\rho_{1p}^2  \right ) - { \sigma}_{p}^2 \left ( 1 - \rho_{1p}^2  \right )  \geq \frac{\epsilon}{(K-1)}, \C \right )\\
    &\qquad + \P \left( \C^c \right).  
\stepcounter{equation}\tag{\theequation}\label{eq:allinone-main}
\end{align*}
The first term on the RHS  above can be bounded as follows:
\begin{align*}
&\P \left ( {\hat \sigma}_{2}^2 \left ( 1 - \hat\rho_{12}^2  \right ) - { \sigma}_{2}^2 \left ( 1 - \rho_{12}^2  \right ) \geq \frac{\epsilon}{(K-1)}, \C  \right )\\
 %%%%%%%%%%%%%%%%%%%%%%%
 &\le \P \left (  \rho_{12}- \hat\rho_{12} \geq \frac{\epsilon}{4(K-1)(1+\eta)}, \C  \right )\\ 
&\qquad + \P \left (  \hat\sigma_{2}^2 - \sigma_{2}^2   \geq \frac{\epsilon}{2(K-1)}  \right ). 
\end{align*}
The proof proceeds by applying concentration results for sample variance, sample standard deviation and sample correlation coefficients to bound the RHS above. The rest of the terms on the RHS of \eqref{eq:allinone-main} are handled in a similar fashion. The reader is referred to Appendix \ref{sec:proofs-mse-conc} for further details.
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection*{Proof of Theorem \ref{thm:lower-bd} \textit{(Sketch)}}
\begin{proof}
% % We follow the technique from \cite{carpentier2016tight} for establishing the lower bound. However, our setting involves correlated arms, with the correlation factors appearing in the mean-square error objective. More importantly, instead of the translation of the mean of sub-optimal arms performed in \cite{carpentier2016tight}, we swap the variances of a pair of arms to interchange the MSE of a sub-optimal arm with that of the optimal arm. %The transformation impacts the variances of all the arms, unlike the classic bandit problem where one could change the mean of a sub-optimal arm in a standalone manner.

Consider problem $m$ with underlying covariance matrix $\Sigma_m$. 
For $(i,j) \in  \S$, let $\nu_{i}\nu_j$ and $\nu_{i}' \nu_j'$ denote bivariate normal distributions with variance and correlations specified by $\Sigma_1$ and $\Sigma_i$, respectively. 
% In particular, the underlying variances are $\sigma_i^2, \sigma_j^2$ for $\nu_i \nu_j$ and $\sigma_i'^2, \sigma_j'^2$ for $\nu_i' \nu_j'$.
Let $\kl_{ij}^m\triangleq KL( \nu_i \nu_j || \nu_i' \nu_j' )$ denote the Kullback-Leibler divergence between $\nu_{i}\nu_j$ and $\nu_{i}' \nu_j'$, where the latter distributions are derived from $\cG_m$. 

If $\rho^2 \le \frac{2K-5}{2K-4}$, we have the following bound for $j=3,\ldots,K$:
\begin{align*}
\kl^2_{1j} & = \frac{1}{2} \left( \frac{2(1-\rho^3)}{1-\rho^4}  - 2  + ln \frac{1-\rho^4}{1-\rho^2} \right)\\
% &\le \frac{\rho^2}{2} \frac{(1-2\rho + 2 \rho^2 - \rho^4)}{1-\rho^4}  \\
& \leq \frac{\rho^2}{2}= \frac{\rho^2 (1-\rho^2)(K-2) }{2 (1-\rho^2)(K-2)} 
% & \leq \frac{\Delta_2}{2 (K-2) r_{12}} \\
% & \leq \frac{\Delta_2}{r_{12}}.
  \le \Delta_2.% \stepcounter{equation}\tag{\theequation}\label{eq:kl-ub-in-lb}
\end{align*}
Along similar lines, we can infer that (see Appendix \ref{sec:appendix-lower-bd})
\begin{align}
 & \max\{\kl^m_{1m},\kl^m_{1j},\kl^m_{mj}, \ j\ne 1,m\} \leq  \Delta_m. \label{eq:kl-bound-lb}
\end{align}
For $(i,j) \in \S$, let $N_{ij}$ denote the number of samples obtained from the joint distribution of $(X_i,X_j)$. 
Let $n_{ij} = \E_{1} N_{ij}$, for $(i,j) \in \S.$
Observe that  
 \\[0.5ex]
\centerline{$\sum\limits_{(i,j) \in \S} N_{ij} = \sum\limits_{(i,j) \in \S} n_{ij} = n. $}
% \[\sum\limits_{(i,j) \in \S} N_{ij} = \sum\limits_{(i,j) \in \S} n_{ij} = n. \]

Notice that the problem transformations impact the distribution of each arm and hence, we cannot employ a change of measure identity similar to \cite{audibert2010best}. 
Instead, we factor in the KL-divergences $\kl_{ij}, \ \forall \ (i,j) \in \S$ and derive a change of measure identity as follows:  for any measurable event $\cE$ based on the samples, 
\begin{align*}
\P_{m}(\cE) &= \E_{\nu_1 \cdots \nu_K}\left[\mathbf{1}\{\cE\} \prod\limits_{(i,j) \in \S} \prod\limits_{s \in {\cal T}_{ij}(n)}\frac{ d \nu_{i}' \nu_{j}' }{d \nu_{i} \nu_{j}}(X_{i,s}, X_{j,s})\right]\\
& = \E_{\nu_1 \cdots \nu_K}\left[\mathbf{1}\{\cE\}\exp\left(\sum\limits_{(i,j)\in\S} -N_{ij}\ekl_{ij,N_{ij}}\right)\right] \\
& = \E_{1}\left[\mathbf{1}\{\cE\}\exp\left(\sum\limits_{(i,j)\in\S} -N_{ij}\ekl_{ij,N_{ij}}\right)\right], 
\end{align*}
where ${\cal T}_{ij}(n)$ is the set of time instants when the algorithm pulled the tuple $(i,j)$. %Further, $\nu_1' \nu_2' \nu_3'$ translate into one of the problem transformations specified earlier and hence $\E_{\nu_1' \nu_2' \nu_3'}=\E_m$.
% as the product distributions $\mathcal G^i$ and $\mathcal G^1$ only differ in $i$ and as the active strategy only explored the samples $(X_{k,s})_{k \leq K, s \leq N_k}$.
For $(i,j) \in \S, 1\leq t\leq n$, let 
%$$\ekl_{(ij),t} = \sum \limits_{s=1}^{t} \log \frac{ d \nu_{i} \nu_{j} }{d \nu_{i}' \nu_{j}'}(X_{i,s}, X_{j,s}) ,$$
\begin{align*}
  \ekl_{ij,t}  &= \frac{1}{t} \sum \limits_{s=1}^{t} \log \frac{ d \nu_{i} d \nu_{j} }{d \nu_{i}' d \nu_{j}'}(X_{i,s}, X_{j,s}) %\\
%  &= \frac{1}{2t} \sum \limits_{s=1}^{t} [X_{i,s} \ X_{j,s}] ( \Sigma_{(i,j),1}^{-1} - \Sigma_{(i,j),m}^{-1}) \left[\begin{array}{c}
% 	X_{i, s} \\
% 	X_{j, s}  
% \end{array}\right]  +\frac{1}{2} ( \log | \Sigma_{(i,j),m}| -  \log | \Sigma_{(i,j),1} | ),
\end{align*}
where $(X_{i,s},X_{i,s}) $ are i.i.d. $\sim \cG $ for all $s \leq t.$ Here, $\Sigma_{(i,j),m}$ is the covariance matrix of $X_{i}, X_{j}$ for problem $m$, and is a submatrix of $\Sigma_{m}.$
% Notice that the change of measure is from $\nu_1',\ldots,\nu_K'$ to $\nu_1,\ldots,\nu_K$, where the transformed distributions $\nu_i'$ are governed by the correlation matrix $\Sigma_m$. 
% Thus, the distributions of $\nu_{i}', \nu_{j}'$ in the definition of $\ekl_{ij,t}$ are to be interpreted as coming from the appropriate bivariate distribution in $\cG_m$.
Let $
\xi = \Big\{\forall (i,j) \in \S, 1\leq t\leq n, \ekl_{(ij),t}  - \kl_{ij}\leq \tilde \epsilon_t \Big\},
$
where $\tilde \epsilon_t$ is as defined in the theorem statement.
Then, for $m=1,\ldots,K$,
$\P_{m}(\xi) \geq 5/6$, which implies that the  empirical divergences concentrate (see Lemma \ref{xi} in the appendix for a proof).

Now, considering algorithms that satisfy $\mathbb E_{1}(\hat A_n \neq 1) \leq 1/2$, we obtain
% . 
% Then, $\mathbb P_{1} (N_{ij} \geq 6 n_{ij}) \leq \frac{\mathbb E_1 N_{ij}}{6n_{ij}} = 1/6$ by Markov inequality. 
% Thus, we have 
% $$\mathbb P_{1}(\mathcal E) \geq 1 - (1/6+1/2 +1/6) = 1/6.$$  
% Using the equation above and \eqref{eq:event1}, we obtain
\begin{align*}
\P_{m}(\hat A_n \neq m)  &\geq \frac{1}{6}\exp\Big(-\sum\limits_{(i,j)\in\S}6n_{ij}\kl^m_{ij} -{K \choose 2} n\tilde \epsilon_{n}\Big)\\
&\geq \frac{1}{6}\exp\Big(-\sum\limits_{(i,j)\in\S}6 n_{ij}\Delta_m -{K \choose 2} n\tilde \epsilon_{n}\Big),
\end{align*}
where the  final inequality follows from the bounds on $\kl^m_{ij}$ above.

% \begin{align*}
%  \sum \limits_{i \neq j} n_{ij} = n.
% \end{align*}
Let $l_{i} = n_{12} + \ldots n_{1K} + \sum \limits_{i \neq 1,i} n_{ij}$. Then, there exists an $i$ such that
$
l_{i }  \leq  \frac{n(K-1)}{H_{lb} \Delta_i}, 
$
where $H_{lb}$ is as defined in the theorem statement.
 If not, then we obtain a contradiction (see Appendix \ref{sec:appendix-lower-bd} for a rigorous justification).
For the aforementioned $i$, from \eqref{eq:final} we have 
\begin{align}
&\P_{m}(\hat A_n \neq m)  \geq \frac{1}{6}\exp\Big(- \frac{6 nK}{H_{lb}} -{K \choose 2} n\tilde \epsilon_{n}\Big).\label{eq:final1-main}
\end{align}
The main claim follows.
\end{proof}

